Fast and Attributed Change Detection on Dynamic Graphs with Density of States

How can we detect traffic disturbances from international flight transportation logs or changes to collaboration dynamics in academic networks? These problems can be formulated as detecting anomalous change points in a dynamic graph. Current solutions do not scale well to large real-world graphs, lack robustness to large amounts of node additions/deletions, and overlook changes in node attributes. To address these limitations, we propose a novel spectral method: Scalable Change Point Detection (SCPD). SCPD generates an embedding for each graph snapshot by efficiently approximating the distribution of the Laplacian spectrum at each step. SCPD can also capture shifts in node attributes by tracking correlations between attributes and eigenvectors. Through extensive experiments using synthetic and real-world data, we show that SCPD (a) achieves state-of-the art performance, (b) is significantly faster than the state-of-the-art methods and can easily process millions of edges in a few CPU minutes, (c) can effectively tackle a large quantity of node attributes, additions or deletions and (d) discovers interesting events in large real-world graphs. The code is publicly available at https://github.com/shenyangHuang/SCPD.git

==> 060discussion.tex <==
\section{Discussion}

% Both \method and \newmethod models the changes in the distribution of singular values of the Laplacian. As shown in Table~\ref{tab:results}, \newmethod can correctly detect change points in large scale dynamic graphs and even outperforms \method in BA-5k experiment. As \newmethod is an approximation method, and it is still more accurate to compute the exact SVD for small graphs~(i.e. number of nodes smaller than 1000). For large graphs, the DOS captures the distribution of singular values as a form of spectral signature~\cite{dong2019network}. When compared to \method, \newmethod achieves equal or better performance with only 1.0\% and 0.7\% of the computational time on SBM-5k and BA-5k experiment respectively. 

% %what information is lost when going from LAD to DOS
% Recently, Rubin~\cite{rubin2020manifold} showed that the spectral embedding of existing random graph models including graphons and other latent position models should live close to a one-dimensional structure. This suggests that the spectrum of an arbitarily large graph sampled from a random graph model could be embedded into a low dimensional vector. As shown in Figure~\ref{Fig:SBM.change} and~\ref{Fig:BA.change}, the change in the distribution of singular values correspond closely to changes in the generative model. Therefore, the DOS could be a natural way to obtain the aforementioned low dimensional embedding. One promising future direction would be to examine how the distribution of singular values of the Laplacian matrix corresponds to parameter changes in the random graph model. 
